Sample Complexity Bounds for Recurrent Neural Networks with Application to Combinatorial Graph Problems

Learning to predict solutions to real-valued combinatorial graph problems promises efficient approximations. As demonstrated based on the NP-hard edge clique cover number, recurrent neural networks (RNNs) are particularly suited for this task and can even outperform state-of-the-art heuristics. However, the theoretical framework for estimating real-valued RNNs is understood only poorly. As our primary contribution, this is the first work that upper bounds the sample complexity for learning real-valued RNNs. While such derivations have been made earlier for feed-forward and convolutional neural networks, our work presents the first such attempt for recurrent neural networks. Given a single-layer RNN with $a$ rectified linear units and input of length $b$, we show that a population prediction error of $\varepsilon$ can be realized with at most $\tilde{\mathcal{O}}(a^4b/\varepsilon^2)$ samples. We further derive comparable results for multi-layer RNNs. Accordingly, a size-adaptive RNN fed with graphs of at most $n$ vertices can be learned in $\tilde{\mathcal{O}}(n^6/\varepsilon^2)$, i.e., with only a polynomial number of samples. For combinatorial graph problems, this provides a theoretical foundation that renders RNNs competitive.

==> images/data.tex <==
\begin{figure}[h]
	

	\centering
	\begin{minipage}{0.3\textwidth}
		\includegraphics[scale = 0.15]{images/testgraph_sparse.pdf}
	\end{minipage}
	\begin{minipage}{0.3\textwidth}
		\includegraphics[scale = 0.15]{images/testgraph_medium.pdf}
	\end{minipage}
	\begin{minipage}{0.3\textwidth}
		\includegraphics[scale = 0.15]{images/testgraph_dense.pdf}
	\end{minipage}
	\caption[Examplary ER graphs with 10 vertices and distinct densities.]{Examplary ER graphs with 10 vertices and edge probabilities $p=0.1$ (sparse graphs), $p=0.5$ (medium dense graphs), and $p=0.9$ (dense graphs).}
	\label{fig:expgraphs}

\end{figure}
